Open-domain Question Answering via Chain of Reasoning over Heterogeneous Knowledge

We propose a novel open-domain question answering (ODQA) framework for answering single/multi-hop questions across heterogeneous knowledge sources. The key novelty of our method is the introduction of the intermediary modules into the current retriever-reader pipeline. Unlike previous methods that solely rely on the retriever for gathering all evidence in isolation, our intermediary performs a chain of reasoning over the retrieved set. Specifically, our method links the retrieved evidence with its related global context into graphs and organizes them into a candidate list of evidence chains. Built upon pretrained language models, our system achieves competitive performance on two ODQA datasets, OTT-QA and NQ, against tables and passages from Wikipedia. In particular, our model substantially outperforms the previous state-of-the-art on OTT-QA with an exact match score of 47.3 (45 % relative gain).

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}


\newcommand{\R}{\mathbb{R}}

\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mR}{\mathcal{R}}

\newcommand{\iL}{\mathit{L}}
\newcommand{\iQ}{\mathit{Q}}
\newcommand{\iR}{\mathit{R}}
\newcommand{\iU}{\mathit{U}}
\newcommand{\iV}{\mathit{V}}
\newcommand{\iX}{\mathit{X}}
\newcommand{\iY}{\mathit{Y}}

\newcommand{\sigmoid}{\text{sigm}}
%\newcommand{\vector}{\text{vec}}
\newcommand{\KL}{\text{KL}}
\newcommand{\Loss}{\mathcal{L}}
% \newcommand{\st}{\text{ s.t. }}

% Objective functions
\newcommand{\bilinear}[3]{#1^{\top}#2#3}
\newcommand{\bidiag}[3]{(#1 \circ #3) ^{\top} #2}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\biband}[3]{#1^{\top}#2#3}

% Dependency paths
\newcommand{\leftarc}[1]{$\leftarrow${[#1]}-}
\newcommand{\rightarc}[1]{-{[#1]}$\rightarrow$}
\newcommand{\wildcard}{$\langle*\rangle$}

\newcommand{\gene}[1]{{\texttt{#1}}}
\newcommand{\rev}[1]{#1$^{-1}$}

\newcommand{\neigh}[1]{\text{nb}\left(#1\right)}
\newcommand{\diagm}[1]{\text{diag}\left(#1\right)}
\newcommand{\ind}[1]{\mathbf{1}\left(#1\right)}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
%\newcommand{\vector}[1]{\underset{#1}{\text{vec}}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\newcommand{\cheading}[2]{\textbf{#1\hfill #2}}
\newcommand{\highest}[1]{\textbf{#1}}% == highest score



%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
% \newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.3mm]}
\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\etc}{\emph{etc.}\ }
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.,}\ }
\newcommand{\ie}{\emph{i.e.,}\ }
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\rhs}{\text{ r.h.s. }}
\newcommand{\lhs}{\text{ l.h.s. }}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\tauvec}{\vec{\tau}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
\newcommand{\Img}{\ensuremath{\mathrm{Im}}}

\newcommand{\cvxCondjc}{{\sf cvxCondJC}}
\newcommand{\cvxCond}{{\sf cvxCond}}
\newcommand{\altCondjc}{{\sf altCondJC}}
\newcommand{\altCond}{{\sf altCond}}

\newcommand{\cvxDisc}{{\sf cvxDisc}}
\newcommand{\JB}{{\sf JB}}
\newcommand{\GS}{{\sf GS}}

\newcommand{\cvxJoint}{{\sf cvxJoint}}
\newcommand{\LG}{{\sf LG}}
\newcommand{\NB}{{\sf NB}}

%%%%%%%%%%%%%%%%%%%linear algebra defs%%%%%%%%%%%%%%%
\newcommand{\unifint}{\int^{1}_{0}}


==> EMNLP 2022/0-Abstract.tex <==

\begin{comment}
Reasoning step by step over open-domain heterogeneous knowledge sources is a challenging task.
Previous work have focused on symbolic methods for this problem.
Recently, large pretrained language models (PLMs) are found to have certain reasoning capability. 
When elicited with explicit prompts, PLMs can perform systematic reasoning for synthetic cases. 
In this paper, we propose a novel reasoning framework combing the strengths of both streams for open-domain applications.
Specifically, we augment the PLM-based reasoning with discrete operations/modules to perform explicit reasoning, i.e. finding and piecing together relevant evidences from various sources.
We verify the generality of the proposed framework by designing a novel open-domain question answering (ODQA) system against tables and documents.
One notable significance of our approach is that it can naturally handle different inference types (e.g. multi-hop vs single-hop questions, text-only vs multi-modality knowledge), unifying multiple efforts in the literature.
We demonstrate the effectiveness of our method on two popular ODQA datasets, OTT-QA and NQ, in comparison with previous task-specific models.
In particular, our model achieves the state-of-the-art (SOTA) results on OTT-QA by outperforming the previous SOTA by 14+ points on exact match score (40 $\%$ relative gain).
\end{comment}

We propose a novel open-domain question answering (ODQA) framework for answering single/multi-hop questions across heterogeneous knowledge sources.
The key novelty of our method is the introduction of the intermediary modules into the current retriever-reader pipeline.
Unlike previous methods that solely rely on the retriever for gathering all evidence in isolation,
our intermediary performs a chain of reasoning over the retrieved set.
Specifically, our method links the retrieved evidence with its related global context into graphs and organizes them into a candidate list of evidence chains.
Built upon pretrained language models, our system achieves competitive performance on two ODQA datasets, OTT-QA and NQ, against tables and passages from Wikipedia.
In particular, our model substantially outperforms the previous state-of-the-art on OTT-QA with an exact match score of 47.3 (45 $\%$ relative gain). \blfootnote{$\dagger$ Part of this work is done during an internship at Microsoft Research} \blfootnote{$*$ Equal contribution}

==> EMNLP 2022/1-Introduction.tex <==
\section{Introduction}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.65]{EMNLP 2022/intro.png}
%     \caption{An illustration of previous single-hop retriever (left) and multi-hop retriever (right) models, where grey dot represent question, blue dots represents retrieved documents in first hop and purple dots are retrieved documents in second hop.}
%     \label{fig:intro}
% \end{figure}


The task of open-domain question answering (ODQA) typically involves multi-hop reasoning, such as finding relevant evidence from knowledge sources, piecing related evidence with context together, and then producing answers based on the final supportive set.
While many questions can be answered by a single piece of evidence \cite{joshi-etal-2017-triviaqa,kwiatkowski-etal-2019-natural},
answering more complex questions are of great interest and require reasoning beyond \textit{local} document context \cite{yang-etal-2018-hotpotqa, geva-etal-2021-aristotle}.
The problem becomes more challenging when evidence is scattered across heterogeneous sources, \eg unstructured text and structured tables \cite{chen2020open}, which necessitates hopping from one knowledge modality to another. 
Consider the question in \autoref{fig:model}.
To form the final answer, a model needs to find the entry list (a table) of the mentioned touring car race, look up the driver name with the correct rank, search for the corresponding driver information, and extract the birthplace from the free-form text.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{concept.png}
    \caption{Our \ourmodel\ vs. previous retriever-only methods for evidence discovery. The grey square is the question, the blue dots are 1st-hop passages, the blue triangles are 1st-hop tables, and the purple dots are 2nd-hop passages.}
    \label{fig:concept}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[scale=0.48]{model.png}
    \caption{An illustration of \ourmodel\ for ODQA. 
    Given a question, the \textit{retriever} first finds hop-1 evidence from the entire Wikipedia (orange arrows). 
    Then the \textit{linker} gathers relevant documents for the hop-1 evidence (purple arrows), which are treated as hop-2 evidence.
    Next, the \textit{chainer} reranks all hop-1 and hop-2 evidence and splices them together into evidence chains (blue arrows).
    Finally, the \textit{reader} takes in the top-50 chains and produces the answer (black arrows).
    The gold evidence chain is marked in red.}
    \label{fig:model}
\end{figure*}

Existing \textit{retriever-reader} methods \citep[][\textit{inter alia}]{min2021neurips} for ODQA mainly customize the retriever model for tackling individual question types, \ie exclusively relying on the retriever to gather all necessary context in a query-dependent fashion.
As shown in \autoref{fig:concept}, the single-hop model \cite{karpukhin-etal-2020-dense} only retrieves a list of isolated passages (blue dots).
For multi-hop cases, an iterative retriever looks for a query-dependent path of passages (blue-purple dot chains) \cite{xiong2020answering}, \ie the later hop passages are retrieved using expanded queries including the original question and previous hop passages.
Although those retrieval-only methods achieve promising results on their targeted cases, the customized retrievers are unable to generalize well.
For example, an iterative passage retriever trained with both multi-hop and single-hop questions performs poorly over both types \cite{xiong2020answering}.
For real-world applications with heterogeneous knowledge sources, it is desirable for an ODQA system to handle both cases well, and the retrieval-only methods are unlikely to succeed.





% In this paper,
We propose a novel \textbf{C}hain \textbf{O}f \textbf{RE}asoning (\ourmodel) framework that generalizes well on both single-hop and multi-hop question answering.
The main contribution of \ourmodel\ is the introduction of two intermediary modules, the linker and the chainer, that play the bridging role between the retriever and the reader, \ie 
piecing together related evidence with necessary context for single/multi-hop questions.
These two modules work in a forward-backward fashion.  
In the forward pass, the linker, a novel table entity linking model (\S\ref{subsec:linker}), links the raw evidence with its related context (\eg table-passage graphs in \autoref{fig:concept}). 
The chainer, a new unsupervised reranker (\S\ref{subsec:chainer}), then prunes all linked evidence using the corresponding question generation scores from a pretrained language model \cite{sanh2021multitask} to form a shortlist of relevant evidence chains in a backward noisy channel fashion (\eg table-passage paths in \autoref{fig:concept}).
By delegating the \textit{hopping} operation to the intermediary, our formalization can potentially gather evidence more effectively over different question types.

% When a question comes in, we first retrieve relevant evidence documents using a dense retriever, then we expand the retrieved documents using the edges in the hybrid graph, therefore completing the reasoning chain for complex questions (\S\ref{subsec:chainer}).
% Our reader then jointly reason over the linked evidences to find the final answer. 

To demonstrate the effectiveness of \ourmodel, we evaluated the proposed model on two popular ODQA datasets, the multi-hop dataset OTT-QA \cite{chen2020open} and the single-hop dataset NQ \cite{kwiatkowski-etal-2019-natural}.
Empirically, we show that our approach is general for both types of reasoning in ODQA.
In particular, \ourmodel\ substantially outperforms the previous state-of-the-art (SOTA) on OTT-QA by 14+ points on exact match scores ($45\%+$ relative gain), and it is competitive with SOTA models on NQ. Moreover, we show that one single unified model can learn to solve both tasks under our framework. 
% , validating the effectiveness of approach.
% We also show that when using one unified model to solve both tasks, it outperforms single-dataset model on OTT-QA while matching the sinlge-dataset performance on NQ. \chenghao{sth comes out of analyses.}
From our analysis, we also find that our evidence chains can potentially help answer single-hop questions by enriching the evidence with more supportive context. \footnote{Data and code available at \url{https://github.com/Mayer123/UDT-QA}}

% \chenghao{If short in space, we can cut the summary of contribution too.}
% In summary, the contributions of this work are:
% \begin{itemize}
%     \item a general ODQA framework with intermediary modules to support multi-hop reasoning against heterogeneous knowledge sources;
%     \item a novel and unified ODQA system for answering both multi-hop and single-hop questions over table and passages from Wikipedia;
%     \item new SOTA results on OTT-QA and competitive performance on NQ.
% \end{itemize}

%\section{Intro V1}
%\chenghao{Most of this can go into related work.}
%Open-domain question answering (ODQA) is a challenging task that requires the model to retrieve relevant documents from large-scale corpus and then reason over retrieved evidence to derive the answer \cite{chen-etal-2017-reading,lee-etal-2019-latent}. While many questions can be can be answered by a single piece of evidence \cite{joshi-etal-2017-triviaqa,kwiatkowski-etal-2019-natural}, recent effort have also focused on more complex questions that require reasoning across multiple evidence documents \cite{yang-etal-2018-hotpotqa, geva-etal-2021-aristotle}. The problem becomes even more challenging when the required evidence are scattered across heterogeneous sources, e.g. unstructured text vs structured tables \cite{chen2020open}, as the model needs to learn to hop from one modality of knowledge to another. 

%Previous works on ODQA adopts different modeling methods for solving single-hop or multi-hop questions. For single-hop questions, the model only retrieve once over the document index and the Top-K returned documents are processed by the reader \cite{karpukhin-etal-2020-dense}. Whereas for multi-hop questions, the retriever runs multiple times using the question and documents returned in previous rounds as query, to find the complete reasoning chains \cite{xiong2020answering}. While these methods achieve promising results on their targeted problem sets, they can not generalize well to other types of questions.  

%In this paper, we propose a novel framework that unifies the solutions for single hop and multi-hop questions over heterogeneous sources. In particular, we first build a bipartite graph between different knowledge sources, then our retriever run inference only on one of the knowledge source and we expand the retrieved documents using the edges in the bipartite graph, therefore completing the reasoning chain for multi-hop questions. Our reader then jointly reason over the linked evidences to find the final answer. We evaluated our framework on the multi-hop dataset OTT-QA \cite{chen2020open} and single-hop dataset NQ \cite{kwiatkowski-etal-2019-natural}. Our method achieves the state-of-the-art results on OTT-QA by outperforming the previous SOTA by 14+ points on exact match score, which is over 40\% relative gains.  


==> EMNLP 2022/2-Overview.tex <==
\section{Overview of the \ourmodel\ Framework}
% In this section, we first provide a formal definition of the considered task. 
% Then we present the overview of our system for ODQA.
%An illustration of our framework is shown in \autoref{fig:model}. 

% \subsection{Problem Definition}
The \ourmodel\ framework is designed to answer questions 
where the answer is a contiguous span from a table $t$ or a passage $p$.
% In our task, the model is asked to provide an answer to a question,
% The task we consider requires the model to provide an answer given a question,
% where the answer is a contiguous span from a table $t$ or a passage $p$.
Here neither $t$ nor $p$ is given, so they need to be retrieved from the table corpus $\mathbb{C}_{t}$ and the passage corpus $\mathbb{C}_{p}$, respectively.
For single-hop questions, a single $t$ or $p$ may be sufficient,
whereas for multi-hop questions, one or more $t$ and $p$ are required to find the answer. 

% \subsection{System Overview}
As shown in \autoref{fig:model}, \ourmodel\ consists of a \textit{retriever}, 
a \textit{linker}, a \textit{chainer} and a \textit{reader}. 
We adopt the DPR model \cite{karpukhin-etal-2020-dense} as our retriever.
We only briefly describe the retriever here as it is not the main focus of our work.
The DPR is a bi-encoder model that consists of a question encoder and a context encoder.
For our setting, the questions and passages/tables are represented by the \clstoken~embedding produced by their respective encoder, and the retrieval is done by maximum inner product search in the vector space.
For a given question, we use DPR to retrieve the initial evidence set which includes tables and passages. %Since the tasks we consider always uses tables in first hop, we only run DPR to retriever from $\mathbb{C}_{t}$ given question. 


Given the initial evidence set (\eg the car race entry list table in \autoref{fig:model}), our intermediary module produces a list of query-dependent evidence chains (\eg the red line linked evidence chain consisting of the car race entry list and the driver's Wikipedia page).
We first propose a linker model (\S\ref{subsec:linker}) to expand the candidate evidence set by including extra passages related to tables in the initial set (purple arrows in \autoref{fig:model}).
This step allows the model to enrich the evidence context, especially including reasoning chains needed for multi-hop questions. %In practice, we run linker model as a pre-processing step to link all the documents in the corpus and store all the edges offline, such that the evidence set expansion can be done in a efficient way.  
Since there could be many links between a piece of evidence and others (\ie a densely connected graph), considering all links is computationally infeasible for the downstream reader.
Thus, we develop a chainer model (\S\ref{subsec:chainer}) to prune the evidence graph with the corresponding question and then chain the evidence across hops together to form query-dependent paths.
Here, we only keep top-$K$ scored chains for reading so that the reader can work on a fixed computation budget.

Finally, the Fusion-in-Decoder (FiD) \cite{izacard-grave-2021-leveraging}, a T5-based generative model \cite{raffel2019exploring}, is used as the reader for generating the final answer.
The model first encodes each top-$K$ evidence chain independently along with the question.
During decoding, the decoder can attend to all chains, thus fusing all the input information. % We use FiD to read our set of reasoning chains produced from previous step to generate the final answer. 



==> EMNLP 2022/3-Approach.tex <==
\section{Intermediary Modules}
In this part, we present the two key components of \ourmodel\ for supporting multi-hop reasoning, \ie the linker for building evidence graphs and the chainer for forming query-dependent paths.

\subsection{Linker}
\label{subsec:linker}
%\chenghao{maybe re-writing this part based on comparison to BLINK. No decoration and table-to-passage.}
In this work, we mainly focus on linking an entity mention in the retrieved evidence to the corresponding Wikipedia page for building evidence graphs.
This setup is related to the recent entity linking work \cite{wu-etal-2020-scalable}. However, there are important modifications for ODQA.
In particular, instead of assuming the entity mention as a prior,
we consider a more realistic end-to-end scenario for ODQA: the linker model has to first \textit{propose candidate entity mentions (spans)} for a given evidence
(\eg ``Tony Longhurst'' in \autoref{fig:model}),
and then \textit{links the proposed mention} to its Wikipedia page.
Another major difference is that we study entity mentions in tables instead of text.
As tables contain more high-level summary information than text, using tables as pivots for constructing evidence graphs can potentially help improve the recall of evidence chains for QA. In the meanwhile, this task is challenging due to the mismatch between the lexical form of the table cells and their linked passage titles. For example, the table of "NCAA Division I women's volleyball tournament" contains the cell \textit{VCU}, which refers to \textit{VCU Rams} instead of \textit{Virginia Commonwealth University}. Thus simple lexical matching would not work. 

In the following, we first describe the model for entity mention proposal and then present a novel entity linking model for mentions in tables.
Both models are based on a pretrained language model, BERT \cite{devlin-etal-2019-bert}.
Following previous work \cite{oguz2020unikqa}, we flatten the table row-wise into a sequence of tokens for deriving table representations from BERT.
In particular, we use $x_1, \ldots, x_N$ to denote an input sequence of length $N$.
Typically, when using BERT, there is a prepended token \clstoken~for all input sequences, \ie $\clstoken, x_1, \ldots, x_N$.
Then the output is a sequence of hidden states $\hvec_\clstoken, \hvec_1, \ldots, \hvec_N\in\RR^d$ from the last BERT layer for each input token, where $d$ is the hidden dimension.
\begin{comment}
\noindent \textbf{Task Set-up} Here we make the assumption that tables often contain more condensed information with broad coverage, whereas text usually contains more targeted and fine-grained descriptions. Intuitively, tables can help maximize the recall of evidence to the answer, and text can help fill in any knowledge gaps required for reasoning. Thus we view tables as pivots for constructing reasoning chains and we propose to build a hybrid graph of tables and text passages by linking all relevant text passages to the tables. We cast this step as an entity linking problem, i.e. we try to link all of the entity mentions in the table to passages that describe these entities. 
%Given a table $t$, we find all of the passages that are relevant to the table. 
\end{comment}

\noindent \textbf{Entity Mention Proposal} In realistic settings, the ground truth entity mention locations are not provided.
Directly applying an off-the-shelf named entity recognition (NER) model can be sub-optimal as the tables are structured very differently from the text.
%\chenghao{Do we have quick stats for that?}
Thus, we develop a span proposal model to label the entity mentions in the table.
Specifically, we use BERT as the encoder (\bert\textsuperscript{m}) and add a linear projection to predict whether a token is part of an entity mention for all tokens in the table,
%\chenghao{have we tried fixing the BERT but fine-tune the header only?}
\begin{align}
    \hvec\textsuperscript{m}_1, \ldots, \hvec\textsuperscript{m}_N & = \bert\textsuperscript{m}(t_1, \ldots, t_N), \\
    \hat{\yvec} & = W \hvec\textsuperscript{m},
\end{align}
where $\hvec\textsuperscript{m} \in \RR^{N \times d}$ and $W\in \mathbb{R}^{2 \times d}$.
The model is trained with a token-level binary loss 
\begin{equation}
    -\frac{1}{N}\sum^{n=1}_N
   (y_n \log P(\hat{\yvec})_1  + (1 - y_n)\log P(\hat{\yvec})_0),
   % (\frac{ e^{\hat{\yvec}_i^{y_i}}}{e^{\hat{\yvec}_i^{0}}+e^{\hat{\yvec}_i^{1}}})
\end{equation}
where $y_n$ is the 0-1 label for the token at position $n$, and $P(\cdot)$ is the softmax function.

\noindent\textbf{Table Entity Linking}
Once the candidate entity mentions are proposed, we follow \citet{wu-etal-2020-scalable} to use a bi-encoder model for linking.
Similarly, two BERT models are used to encode tables (\bert\textsuperscript{t}) and passages (\bert\textsuperscript{p}), respectively.
% \noindent \textbf{Architecture} Similar to \cite{wu-etal-2020-scalable}, we employ a bi-encoder model to find these links, consisting of two language model encoders $BERT_t$ and $BERT_p$, one for tables and one for passages respectively.
In contrast, as there are multiple entity mentions for each table, we want to avoid repetitively inserting additional marker tokens and re-computing representations for each mention occurrence.
Accordingly, we cannot simply take the \clstoken~ embeddings for linking as previous work \cite{wu-etal-2020-scalable}.
Inspired by \citet{baldini-soares-etal-2019-matching}, to represent each entity mention, we propose a new entity representation based on the entity start and end tokens.
For an entity mention with a start position $i$ and end position $j$ in the table, we compute our proposed entity embedding $\evec\in\RR^d$ for linking by%\footnote{In our pilot study, we found this setting to work best.}
% first take the average of the start and end embeddings to form the localized entity representation $\evec \in \mathbb{R}^d$, and then compute the final embedding for linking $\qvec$.
\begin{align}
    \evec = & (\hvec\textsuperscript{t}_i + \hvec\textsuperscript{t}_j)/2, %\\
    %\qvec = & (\evec + \hvec\textsuperscript{t}_\clstoken)/2.
\end{align}
% where s and e are start and end indices of the entity mention in the table.
% Then we take the average of $E_{enc} \in \mathbb{R}^d$ with the [CLS] token embedding $t_{enc}^{cls}$ to fuse in the table context information to form $Q_{e} \in \mathbb{R}^d$. $Q_{e}$ is then used as query vector to search through the dense document index to retrieve the linked passages.
%\chenghao{do we have any ablation here? such as e without cls?}
For passages, we directly take the \clstoken~ hidden state $\pvec=\hvec\textsuperscript{p}_\clstoken\in\RR^d$ as the passage representation.
Following the literature, the table entity linker is trained based on a contrastive learning objective
\begin{equation}
      L_\textsubscript{sim} = -{\exp(\text{sim}(\evec, \pvec^+)) \over \sum_{\pvec^\prime\in\mathcal{P}\cup\{\pvec^+\}} \exp(\text{sim}(\evec, \pvec^\prime))},
    \label{eqn:obj_sim}  
\end{equation}
where $\pvec^+$ is the corresponding (positive) passage and $\mathcal{P}$ is the irrelevant set of negative passages.

% \begin{align}
%     t_{enc} = & BERT_t(t) \\
%     p_{enc} = & BERT_p(p)
% \end{align}
% where $t_{enc} \in \mathbb{R}^{N \times d}$. 

\begin{comment}
\noindent \textbf{Entity Mention Modeling} Different from \cite{wu-etal-2020-scalable}, we do not insert any marker tokens to represent the entity mentions, hence all entity mentions from $t$ share the same encoded table representation $t_{enc}$. To represent each individual entity mention, inspired by \cite{baldini-soares-etal-2019-matching}, we propose to use entity start and end token representations. In particular, we take the average of the start and end tokens to form the localized entity embedding $E_{enc} \in \mathbb{R}^d$.
\begin{align}
    E_{enc} = & (t_{enc}^s + t_{enc}^e)/2 \\
    Q_{e} = & (E_{enc} + t_{enc}^{cls})/2
\end{align}
where s and e are start and end indices of the entity mention in the table. Then we take the average of $E_{enc} \in \mathbb{R}^d$ with the [CLS] token embedding $t_{enc}^{cls}$ to fuse in the table context information to form $Q_{e} \in \mathbb{R}^d$. $Q_{e}$ is then used as query vector to search through the dense document index to retrieve the linked passages. On the passage side, we directly take the [CLS] token representation as the passage embedding, denote as $P \in \mathbb{R}^d$. 
\end{comment}

\noindent \textbf{Training}
To train our linker including entity mention proposal and table entity linking, we leverage a small set of Wikipedia tables with ground truth hyperlinks, where each linked mention and the first paragraph of the linked page constitute a positive pair (see \autoref{sec:appendix-training}).
%\chenghao{a pointer to data information is preferred.}
Similar to \citet{wu-etal-2020-scalable}, we use BM25 \cite{bm25} to mine hard negative pairs for each entity mention.
\begin{comment}
 We train our model with contrastive learning objective
\begin{align}
   L = - log(\frac{e^{Q_{e}^T P^+}}{e^{Q_{e}^T P^+} + \sum^{i=1}_n (e^{Q_{e}^T {P^-}^i})})
\end{align}
where $P^+$ is the positive passage and $P^-$ are the paired hard negative passage and other example's passages within the same batch (in-batch negatives).    
\end{comment}




\noindent \textbf{Inference} During inference, we first use the entity span proposal model to label entity mentions in the tables and then run the table entity linking model to link predicted mentions to passages via maximum inner product search \cite{johnson2019billion}. Here, we allow searching over all passages rather than the first paragraph of each Wikipedia page for recall purposes.
% (finding the maximum dot product between entity mention representation and encoded passages). 
For efficient inference, the passage corpus can be pre-computed and stored as done in dense retrieval \cite{karpukhin-etal-2020-dense}. Then we can build links for all tables in the corpus (inducing graph-structured corpus), and directly use the graph to enrich the isolated evidence items from the retriever. 

\subsection{Chainer}
\label{subsec:chainer}
Although the linker model can effectively enrich the table with all relevant passages and provide possible hopping paths for reasoning,
the amount of resulting information is too overwhelming if sent directly for reading, \ie a table could contain multiple entity mentions, resulting in a densely connected evidence graph.
To make it easy for the reader, we use the chainer model to prune graphs and extract the most relevant paths.
Since the linker (\S\ref{subsec:linker}) builds the evidence graphs in a query-agnostic fashion, an important function of chainer here is to incorporate the question when selecting the top-K evidence paths for answer inference.

Motivated by recent work \cite{sachan2022improving} in using pretrained generative language models for passage reranking, we also build the chainer on T0 \cite{sanh2021multitask} in a zero-shot fashion, \ie no training is required.
Different from their approach, we design a novel relevance scoring for query-dependent hybrid evidence path reranking rather than isolated passages.

% \noindent \textbf{Relevance Scoring} 
Given a question $q$, we model the relevance of a question-table-passage path using the following conditional
\begin{align}
    P(t, p|q) = P(p|t, q)P(t|q),
    \label{eqn:relevance_orig}
\end{align}
where $t \in \mathbb{C_T}$, $p \in \mathbb{C_P}$.
The second term $P(t|q)$ is modeled by our retriever. Given that our linker is query-agnostic (\ie only modeling $P(p|t)$), we do not have a good estimation for $P(p|t,q)$ on the right-hand side.
To remedy this, we apply the Bayes rule to \autoref{eqn:relevance_orig}
\begin{equation}
    \label{eqn:relevance_score}
    P(t, p|q) \approx P(q|t, p)P(p|t)P(t|q).
\end{equation}
% As we only consider passages from the linked set and tables from the retrieved set,
% we use the linker score to approximate $P(p|t)$.
To estimate $P(q|t, p)$, we use the question generation likelihood as in \citet{sachan2022improving}. 

Different from \citet{sachan2022improving}, here we have two conditional variables. Naively computing question generation scores on all pairs results in quadratic complexity which is very computation intensive for T0.\footnote{Even the smallest T0 model has 3B parameters.} %\chenghao{have some computation cost estimation would be better, but num of parameters are also good}.
To reduce the inference cost, we further decompose $P(q|t,p)$ into two question generation scores $S_{T0}(q|p)$ and $S_{T0}(q|t)$, both based on the question generation likelihood from T0.
In this way, we can reuse $S_{T0}(q|t)$ for corresponding linked passages with a linear cost.
To compute $S_{T0}(q|p)$ and $S_{T0}(q|t)$, we append the instruction \textit{``Please write a question based on this passage.''}\footnote{Changing ``passage'' to ``table'' in the prompt does not make much difference.}
to every passage/table and use the same mean log-likelihood of the question tokens conditioned on the passage/table  \cite{sachan2022improving}. 

\begin{comment}

To remedy this, we make the assumption that 
\begin{align}
    P(p|t, q) \approx P(p'|q) s.t. p' \in \hat{p}
\end{align}
where $\hat{p}$ is the set of passages linked to t by our linker model. In this case, we can further approximate the right hand side with Bayes rule 
\begin{align}
\label{eq:bayes}
   P(p'|q)\approx P(q|p')
\end{align}
such that $P(q|p')$ can be estimated using a question generation model's loss, which we call Question Generation Score $QGS(q|p')$. 

For the second term on the right hand side, it can be approximated by the score given by our retriever. To further enhance its estimation, we can also use \autoref{eq:bayes} to compute the Question Generation Score for the first-hop evidence to get a more fine-grained relevance score w.r.t the question, $QGS(q|t)$. Note that we also compute Question Generation Score for documents in the first hop that do not have any links, e.g. passages, such that both single documents and linked paths can be reranked together. 
\end{comment}

%For tables or text passages in the initial evidence set, we can also apply the T0 reranker to estimate a more fine-grained relevance score w.r.t the question, denoted as $S(c|q)$ where $c$ represent first hop evidence.
%With all of the scores computed, we experimented with two chaining strategy as following: 

% \noindent \textbf{Score Computation}%  To compute the Question Generation Score for both hops, we adopt the instruction-tuned model T0 following \cite{sachan2022improving}.
% To compute $S_{T0}(q|p)$ or $S_{T0}(q|t)$, we append the following instruction \textit{"Please write a question based on this passage/table."}
% to every passage/table and then use the same average likelihood of the question tokens conditioned on the passage/table as used by \cite{sachan2022improving}. 
% Intuitively, if the passage/table is highly relevant to the question, the model's generation loss should be lower. 


% \noindent \textbf{Chaining Scoring}
%In this case, we reranked the linked chains in one shot and then re-take the Top-K documents/chains. Intuitively, this would allow greater capacity for the linker since the size of the candidate pool for reranking is determined by the number of linked documents. Consequently, it is possible for some top retrieved documents in the first hop to be excluded from the Top-K after reranking. 
As our pilot study suggests that the query-agnostic linker scores are not so informative for query-table-passage paths,
we only combine the retriever score with two question generation scores from \autoref{eqn:relevance_score} as the final chainer score for reranking evidence paths (\ie $P(p|t)$ is dropped)
\begin{equation}
\label{eqn:chainer}
   % CS(t, p'|q) = & -log(\frac{e^{sim(t, q)}}{\sum^{i=0}_D e^{sim(t_i, q)}}) \\
 S_{R}(t, q) + \alpha S_{T0}(q|t) + \beta S_{T0}(q|p),
\end{equation}
where $S_{R}(t, q) \sim P(t|q)$, and is defined as
\begin{equation}
    S_{R}(t, q) = -\text{log} (\frac{\exp(\text{sim}(t, q))}{\sum_{t_i\in\mathcal{T}} \exp(\text{sim}(t_i, q))}),
\end{equation}
$\text{sim}(\cdot, \cdot)$ is the unnormalized retriever score, $\mathcal{T}$ is the first-hop evidence set,
$\alpha$ and $\beta$ are hyper-parameters.
For singleton cases (first-hop table/passage without link), we modify the last two terms of \autoref{eqn:chainer} to $2\alpha S_{T0}(q|t)$ and $2\alpha  S_{T0}(q|p)$ for tables and passages, respectively.
This can help ensure that the chainer scores for singletons and table-passage paths are on the same scale.  %For tables or passages in the initial documents set that do not have links, the third term on the right hand side can not be computed. To make the scores for all the evidence chains on the similar scale, we multiple the second term on the right hand side by 2. 
Then we sort all singletons and chains using the chainer score and keep the top-k results.
We also use heuristics to reduce potential duplication and details are in \autoref{sec:appendix-chain}. 

\begin{comment}
\noindent \textbf{Retriever-oriented} For this setting, we rerank the initially retrieved documents set first then take the top-K. Then we expand the tables in the top-K list by including its one-best linked passage. Intuitively, this strategy allow greater capacity for the retriever since the size of the reranking list is the size of the first-hop documents. Specifically, we use the following chainer score:
\begin{equation}
   CS(c|q) = -log(\frac{e^{sim(c, q)}}{\sum^{i=0}_K e^{sim(c_i, q)}})
    + \gamma S(c|q)
\end{equation}
Then for each table in the Top-K list, we concatenate it with its one-best linked passages given by the reranker score $S(p'|q)$. 
\end{comment}

==> EMNLP 2022/4-Experiments.tex <==
\section{Experiments}
In this section, we first describe datasets and knowledge sources (\S\ref{ssec:datasets}).
Then we discuss single-set and joint-set experiment setups (\S\ref{ssec:exp_setup}) and baselines for comparison (\S\ref{ssec:baselines}).
Finally, we present experiment results on OTT-QA and NQ (\S\ref{ssec:main_results}).

\subsection{Datasets}
\label{ssec:datasets}
\textbf{OTT-QA} \cite{chen2020open} is an open-domain QA dataset that contains mostly multi-hop questions. 
These questions require joint reasoning over evidence from tables and text passages. \\
\noindent \textbf{Natural Questions} (NQ) \cite{kwiatkowski-etal-2019-natural} contains real user queries submitted to the Google search engine and the questions are mostly single-hop and considered solvable using either a single text passage or a table. 
We adopt the open-domain setting proposed by \citet{lee-etal-2019-latent}. 
%\noindent \textbf{NQ-table-answerable} A certain portion of questions in NQ can be answered by a table, and previous work have also specifically explored this subset of questions \cite{herzig-etal-2021-open,wang2022table}. We adopted the same split released by \cite{ma-etal-2022-open} for our experiments.   
%\chenghao{Are we going to report anything on it? if not, we can just comment this out.}

%\subsection{Knowledge Sources}
%\label{subset:know_source}
\noindent For OTT-QA, we adopt its official release of text passages and tables.
The passages are first paragraphs from all Wikipedia pages, whereas tables are well-formed tables from full Wikipedia (\ie no infoboxes, no multi-column/multi-row tables, etc.).
%\chenghao{If short in space, compress it.}
For NQ, we adopt the Wikipedia passage splits from \citet{karpukhin-etal-2020-dense} and we use the processed table sets of full Wikipedia released by \citet{ma-etal-2022-open}.
Statistics can be found in \autoref{sec:appendix-data}.

\subsection{Experimental Settings}
\label{ssec:exp_setup}
%In this section, we describe how we train our models and report end-to-end results on OTT-QA and NQ. 
We train a single \textbf{linker} on the OTT-QA training set, and directly apply it for both tasks. For \textbf{chainer}, we apply the off-the-shelf T0-3B \cite{sanh2021multitask} for reranking on both tasks, \ie no updates to the model. Hence both models are task-independent. %In addition to the realistic setting where we always link tables to passages, we also consider an oralce setting for NQ. Since most of NQ questions only require single-hop reasoning, in the oracle setting we disable linker for NQ and directly use Chainer to rerank retrieved evidence documents. 

%In the default setting, we apply Chainer to the full expanded evidence pools, hence the size of the evidence pool varies for every question. For NQ oracle setting, since there is no link expansion, we increase the initial retrieved set size and apply Chainer to rerank Top500/Top1000 documents.
For both \textbf{retriever} and \textbf{reader}, we consider both \textit{single-set} setup where separate models are trained for individual tasks and the \textit{joint-set} setting where a single model is trained to solve both tasks. 
During inference, the retriever searches over task-specific knowledge sources.
For OTT-QA, since most of its questions have tables as the first-hop evidence, we run the retriever only on the table set in the first hop to find top-100 tables.
For NQ, the retriever searches over the joint index of all text and tables and keeps the top-100 items in the first hop. 
After retrieval, we use the linker to expand tables in the top-100 set into graphs and use the chainer to select the top-50 chains.  
% We instantiate the FiD reader model with T5-Large \cite{raffel2019exploring}.
As the chained evidence is typically longer, unless otherwise specified, we only use the top-50 chains 
and set the maximum sequence length to 500 for the FiD reader. 
More training details are in \autoref{sec:appendix-training}.


\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Dev} & \multicolumn{2}{c}{Test} \\
 & \textbf{EM} &  \textbf{F1} & \textbf{EM} &  \textbf{F1}\\
\midrule
HYBRIDER \cite{chen-etal-2020-hybridqa} & 10.3 & 13.0 & 9.7 & 12.8 \\
FR+CBR\cite{chen2020open}  & 28.1 & 32.5 & 27.2 & 31.5 \\
CARP \cite{zhong2022reasoning} & 33.2 & 38.6 & 32.5 & 38.5 \\
\midrule
Oracle Link + FR+CBR & 35.2 & 39.9 & 35.0 & 39.5 \\
Oracle Link\&table + HYBRIDER & 44.1 & 50.8 & 43.0 & 49.8 \\
\midrule
\ourmodel\, (single) & \bf 49.0 & \bf 55.7 & 46.7 & 53.5 \\
\ourmodel\, (joint) & \bf 49.0 & \bf 55.7 & \bf 47.3 & \bf 54.1 \\
\bottomrule
\end{tabular}
}
\caption{End-to-end QA results on OTT-QA.}
\label{tab:ott_res}
\end{table}

\subsection{Baselines}
\label{ssec:baselines}
We briefly describe the baselines for both tasks.
For OTT-QA, the HYBRIDER \cite{chen-etal-2020-hybridqa} is a reading comprehension model for joint reasoning over tables and passages.
This baseline uses BM25 to retrieve relevant tables and passages.
Instead, Fusion Retriever + Cross-Block Reader (FR+CBR) \cite{chen2020open} first links table rows to passages using BM25 to build an index of linked documents (blocks). Then it trains a biencoder dense retriever (further enhanced by Inverse Cloze Task pretraining \cite{lee-etal-2019-latent}) to find the most relevant blocks. 
Then they use the ETC \cite{ainslie-etal-2020-etc} as the reader to process up to 4K tokens returned by the retriever.
CARP \cite{zhong2022reasoning} employs similar retriever and reader models as FR+CBR, and it additionally extracts hybrid knowledge chains to facilitate the reader's reasoning process. 
All approaches are dataset-specific, hence are unlikely to handle other question types from NQ. We note that both FR+CBR and CARP's reader components adopt models specifically designed for handling long sequences. Since our overall goal is to build a unified system for both single-hop and multi-hop questions, we choose FiD based on its ability to handle different cases. 
We also compare against two oracle settings from \citet{chen2020open}.
The first one uses gold hyperlinks in fusion retriever instead of BM25 to link table rows and passages. 
The second setting adopts gold hyperlinks and gold tables for the HYBRIDER reader, \ie no retrieval is involved.
This setting is previously considered as an estimated upper bound for this task \cite{chen2020open}. 

On NQ, we compare with text-only baselines: DPR \cite{karpukhin-etal-2020-dense} which applies a BERT-based reader to first select the best passage from top-k returned by the retriever and then extracts the answer span in it; FiD \cite{izacard-grave-2021-leveraging}; and UnitedQA \cite{cheng-etal-2021-unitedqa}) which is an extractive model based on ELECTRA \cite{clark2020electra} and enhanced with additional training objectives \cite{cheng-etal-2021-posterior,cheng-etal-2020-probabilistic}.
We also compare with models that consider tables as knowledge sources: Unik-QA \cite{oguz2020unikqa} which augments the document index with NQ tables and uses FiD reader to generate the answer; UDT-QA \cite{ma-etal-2022-open} which incorporates the tables from full Wikipedia and adopts UnitedQA as its reader. 
%\chenghao{Fill in the citations and say a littie bit more about each baseline for NQ.}


\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
 & \textbf{Tables} & \textbf{EM} \\
\midrule
DPR \cite{karpukhin-etal-2020-dense} & N & 41.5 \\
FiD \cite{izacard-grave-2021-leveraging} & N & 51.4 \\
UnitedQA \cite{cheng-etal-2021-unitedqa} & N & 51.8 \\
\midrule
Unik-QA \cite{oguz2020unikqa} & Y & 54.1 \\
UDT-QA \cite{ma-etal-2022-open} & Y & \bf 54.7 \\
\midrule
\ourmodel\, (single) & Y & 54.6 \\
\ourmodel\, (joint) & Y & 53.9\\
\bottomrule
\end{tabular}
}
\caption{End-to-end QA results on NQ test.}
\label{tab:nq_res}
\end{table}


\subsection{Results}
\label{ssec:main_results}
The end-to-end results on OTT-QA are shown in \autoref{tab:ott_res}. 
Our \ourmodel\,models substantially outperform all baselines by a large margin, illustrating the effectiveness of our proposed framework.
It is worth noting that our model also outperforms two oracle settings proposed in \citet{chen2020open}.
This is potentially because the capacity of their reader models is quite limited compared to ours.
For FR+CBR, the model can only read up to 4K tokens, whereas in our case, the FiD reader can process up to 25K tokens.
We also observe that evidence to questions in OTT-QA can be found in many different reasoning chains.
In other words, tables that are not annotated as gold may still provide valuable information for reasoning.
However, only one table is considered in their oracle experiment with HYBRIDER.
Also, it is worth noting that the joint model outperforms the single model on OTT-QA, indicating that our framework can effectively leverage NQ data to benefit OTT-QA.

\autoref{tab:nq_res} summarizes the results on NQ.
Similar to previous work using tables as the extra knowledge source, we also find our method to be consistently better than text-only baselines. 
Overall, \ourmodel\ achieves competitive performance compared to SOTA models. 
It is also worth noting that both Unik-QA and UDT-QA use the iterative training strategy for the retriever, which leads to higher retriever performance. In particular, UDT-QA achieves 91.9 recall@100 on the NQ test set, whereas we only get 90.3. This difference in retriever recall likely explains the gap in the end-to-end QA performance.  
Since iterative training of the retriever is not used by baselines on OTT-QA, we leave that out in our experiments. For consistency, we only train our retriever for one round. Also, we note that the joint model performs slightly worse than the single-dataset model, which is different from the trend observed on OTT-QA. We hypothesize that this is due to the distribution difference of the evidence chains in the two datasets. Most of the top-ranked evidence are chained cases on OTT-QA, whereas that reduces to only 30\% on NQ (the rest 70\% are singleton cases). The current FiD reader may have a hard time reasoning over both singleton and chained cases simultaneously. We leave further exploration for future work. 

==> EMNLP 2022/5-Results.tex <==
\section{Analysis}
In this section, we conduct ablation studies and analyze different components of our framework.

\subsection{Ablation Study}
\begin{table}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 & \textbf{\#Docs} &  \textbf{Max Length} & \textbf{EM} \\
\midrule
\ourmodel\, (single) & 50 & 500 & 49.0  \\
no QGS of hop1 & 50 & 500 & 45.1  \\
no QGS of hop1 & 100 & 300 & 44.8\\
no QGS of hop1\&2 & 100 & 300 & 38.7  \\
no Chainer & 100 & 300 & 29.1 \\
\bottomrule
\end{tabular}
}
\caption{Chainer ablation on OTT-QA dev.}
\label{tab:ott_ablation}
\end{table}
We start by ablating our chainer on the OTT-QA task using \ourmodel\,(single) from \autoref{tab:ott_res}.
The results are summarized in \autoref{tab:ott_ablation}.
First, we experiment with
\textbf{removing question generation score (QGS) for hop1 evidence} (row 2).
In this case, \autoref{eqn:chainer} will not have the second term and a large performance drop is observed, suggesting that it is important to apply chainer to reweight the retrieved items.
Under the same setting, we try to increase the number of items and decrease the max sequence length for reading (row 3).
Here we are interested in seeing the impact of reading more chains while constraining the length of individual chains.
The slight performance drop indicates that potential information loss from longer chains is detrimental to the final performance. 

Then we test \textbf{removing QGS entirely} (row 4).
As there is no reranking at all, we simply take all linked passages for each table based on the initial retrieved order.
Here, since we exhaustively include all linked passages for each table, the reader budget can be quickly filled by the top few retrieved tables, which probably makes the reader suffer from information loss with too many irrelevant items.
Indeed we see another large drop in the QA performance, showing the importance of reranking.
Finally, we experiment with \textbf{removing chainer} (row 5).
It goes one step further by not concatenating the table rows with linked passages and only passing each piece of evidence independently.
Here we are interested in whether FiD is able to fuse the information without explicit chaining.
The largest performance drop is observed here, suggesting that chaining the items from different hops is vital for the reader. 

We also study the effect of the number of retrieved items as input to the reader on its QA performance by varying \textbf{the number of chains sent to the reader}.
The results on OTT-QA dev set are shown in \autoref{tab:ott_res_length}.
As we can see, when reading only the top 10 chains (much less than 4K tokens on average considered by previous work \cite{chen2020open,zhong2022reasoning}), \ourmodel\ still outperforms the previous SOTA method by a large margin, further validating the effectiveness of our framework.
In summary, the reader performance increases with more items, and we hypothesize that the reader can be further improved when given a larger capacity.
We leave this exploration for future work.


\begin{table}[t!]
\centering
%\resizebox{\linewidth}{!}{
\small
\begin{tabular}{lccc}
\toprule
 \textbf{\# Docs} & \textbf{Avg \# Tokens} & \textbf{EM} &  \textbf{F1}\\
\midrule
 50 & 11,897 & \bf 49.0 & \bf 55.7 \\
 20 & 4,757 & 44.9 & 51.8 \\
 10 & 2,351 & 40.8 & 47.0 \\
\bottomrule
\end{tabular}
%}
\caption{Reader ablation with different number of documents on OTT-QA dev.}
\label{tab:ott_res_length}
\end{table}


\subsection{Impact of Linker \& Chainer}
We measure evidence recall scores of our joint model to better understand the impact of the linker and the chainer.
On OTT-QA, since most questions require multi-step reasoning, we evaluate the retriever by both gold cell recall and answer recall.
Here the gold cells refer to table cells whose gold linked passage contains the answer.
We consider a table chunk to be gold if it contains at least one gold cell.
For answer recall, we use top-K chains produced by the chainer.
Since OTT-QA official test set is hidden, we only report dev set results in \autoref{tab:ott_retri}.
As expected, the answer recall scores are extremely low without the linker and chainer,
as most OTT-QA questions are multi-hop and the answers are likely to appear in the hop-2 passages.
To verify if the retriever itself is able to discover the full reasoning chain, we further allow the retriever to search through the joint index of tables and passages (last row).
Compared with the first row, there is some improvement.
On the other hand, with the help of the linker and chainer (row 2), AR@20 and AR@50 
are substantially improved, which also explains our superior QA performance.
We also observe similar trends on NQ, and more results and discussion are in Appendix~\ref{subsec:appendix-linker-chainer}. 

\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & \textbf{R@20} &  \textbf{R@100} & \textbf{AR@20} &  \textbf{AR@50}\\
\midrule
Joint Retriever & \bf 83.8 & \bf 92.1 & 31.8 & 37.6 \\
+Linker\&Chainer & 83.5 & 90.8 & \bf 74.5 & \bf 82.9 \\
\midrule
Retrieve full index & 82.4 & 90.6 & 34.6 & 42.6 \\
\bottomrule
\end{tabular}
}
\caption{Evidence recall of the joint retriever on OTT-QA dev set, where R@K evaluates gold table chunk recall and AR@K evaluates answer recall.}
\label{tab:ott_retri}
\end{table}


\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & \textbf{\# Link} & \textbf{\# No Link} & \textbf{AR@20} &  \textbf{AR@50}\\
\midrule
 \ourmodel\, & 2,214 & 0 & 74.5 & 82.9 \\
 Classifier & 2,133 & 81 & 73.3 & 81.9 \\
 \midrule
 \ourmodel\, & 8,757 & 0 & 85.7 & 88.1 \\
 Classifier & 370 & 8,387 & 86.0 & 88.1 \\
\bottomrule
\end{tabular}
}
\caption{Answer recall on OTT-QA (top) and NQ (bottom) dev with different linking strategies.}
\label{tab:q_type}
\end{table}

\begin{table*}[h!]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ll}
\toprule
 \textbf{Q\&A}& \textbf{Evidence Chain} \\
\hline
\textbf{Q:} who plays ryders mum & \textbf{Table Title:} List of Home and Away characters \\
on home and away & || character, actor(s), duration || \textit{ryder jackson}, lukas radovich, 2017- || \textit{Ryder Jackson} is  \\
\textbf{A:} Lara Cox & a fictional character from the Australian television soap opera "Home and Away" ... \\
 & \textbf{His mother is Quinn Jackson (Lara Cox)}, who is estranged from Alf. When ...\\
\midrule
\textbf{Q:} what was blur 's first & \textbf{Table Title:} List of UK top-ten singles in 1994 \\
number one single in the uk & || artist, weeks, singles || blur, 3, \textit{"girls \& boys"}, "parklife" || \textit{Girls \& Boys} (Blur song) is a 1994 \\
\textbf{A:} Country House & song by British rock band Blur. It was released ... "Girls \& Boys" was Blur's first top 5 hit and \\
& their most successful single until \textbf{"Country House" reached number 1} the following year ... \\
\midrule
\textbf{Q:} Who is the dad of the cyclist  & \textbf{Table Title:} Holland Hills Classic \\
that placed directly behind & || Year, First, Second, Third || 2011, Marianne Vos, Marieke van Wanroij, \textit{Jessie Daams} || \\
Marieke van Wanroij at the & \textit{Jessie Daams} Jessie Daams ( born 28 May 1990 ) is a Belgian racing cyclist . \\
2011 Holland Hills Classic ? & She competed in the 2013 UCI women 's road race in Florence .  \\
\textbf{A:} Hans Daams & \textbf{Her father is the Dutch cyclist Hans Daams} . \\
\midrule
\textbf{Q:} What other team did the& \textbf{Table Title:}  2012 Charlotte Eagles season \\
Cuban player on the 2012 Char- & || No, Position, Player, Nation || 19, Midfielder, \textit{Miguel Ferrer}, Cuba || \textit{Miguel Ferrer} \\
lotte Eagles team play for ?  & (footballer) Miguel Ferrer ( born March 28 , 1987 ) is a Cuban footballer who \textbf{played for} \\
\textbf{A:} Wichita Wings & \textbf{the Wichita Wings} in the Major Indoor Soccer League . \\
\bottomrule
\end{tabular}
}
\caption{Example evidence chains found by our \ourmodel, where || separates tables and passages. The answer evidence is \textbf{bold} and the linked entity mention in the table is \textit{italic}. The first two are from NQ and the latter are from OTT-QA.}
\label{tab:cases}
\end{table*}

\subsection{Alternative Linking Strategy}
Since most NQ questions only require single-hop reasoning,
one alternative linking strategy for NQ is to skip the linker for single-hop ones.
As the question type is typically unknown in real cases,
we experiment with training a question classifier to predict whether a question requires multi-step reasoning or not.
We directly use the encoded question representation produced by our joint retriever, and train a linear classifier for this task.
For simplicity, we consider all NQ questions to be single-hop and all OTT-QA questions to be multi-hop.
Based on this, the classifier can achieve 95.9\% accuracy on the combined dev set of NQ and OTT-QA.
We then proceed to compute answer recall for both NQ and OTT-QA using the classifier to decide 
the linking strategy for each question.
The results are shown in \autoref{tab:q_type}.
We observe the difference in answer recall between \ourmodel\ and that using the question classifier 
is quite small.
Thus, future work can also use this strategy for handling different types of questions.
%Finally, we study the performance of using the linker as a standalone module and find it outperforms previous baselines (Appendix \ref{subsec:appendix-linker}).


\input{6-Analysis}

==> EMNLP 2022/6-Analysis.tex <==


\subsection{Linker Performance}
\label{subsec:appendix-linker}
The success of our framework depends on the linking quality, thus we also evaluated our linker model as a standalone module to better understand its performance. Here we use the 789 tables in the OTT-QA dev set with ground truth hyperlinks for evaluation. For metrics, we compute precision, recall and F1 score for finding all the links for each table and only consider the top-1 retrieved results in all settings. We compare the cell linker model proposed by \citet{chen2020open} as a baseline. In this model, they first train a GPT-2 \cite{radford2019language} model on OTT-QA training set to generate queries for every cell in the table (empty if the model decides to not link a certain cell), and then use BM25 to retrieve passages. In addition, we also consider a baseline that uses ground truth table cells (cells that have links) as queries and retrieve with BM25. The results are shown in \autoref{tab:ott_dev_link}. Our linker achieves the best F1 score compared to the two baselines, and the advantage on recall is especially prominent. The oracle+BM25 model has the best precision because the information for whether a cell requires linking is given as a prior. However, it cannot retrieve well when the passage title does not overlap significantly with the cell text, as discussed in (\S\ref{subsec:linker}). The GPT2 model can alleviate this issue to some extent by generating additional terms for matching, however, it still lags behind our proposed linker model. 

\begin{table}[hbt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 & \textbf{Precision} &  \textbf{Recall} &  \textbf{F1}\\
\midrule
Oracle cell + BM25 & \bf 61.7 & 51.0 & 55.9 \\
GPT2+BM25 & 59.9 & 58.3 & 59.1 \\
Our Linker & 60.3 & \bf 63.0  & \bf 61.6 \\
\bottomrule
\end{tabular}
}
\caption{Linker variants on OTT-QA Dev set tables. In total, there are 20,064 unique passages attached to these 789 tables}
\label{tab:ott_dev_link}
\end{table}


\subsection{Case Study}
We manually inspect evidence chains found by our model to better understand the benefits of our intermediary modules.
Examples where predicted chains contain supportive evidence are in \autoref{tab:cases}. % (more examples in Appendix \ref{subsec:appendix-exp}).

Despite that NQ questions are usually short and single-hop, we posit that some questions can potentially benefit from the proposed chain of reasoning.
As illustrated by the first two examples, though the entity mentions from the tables are not directly relevant, the table-passage chains actually contain the supportive information.
Therefore, in contrast to considering the evidence in isolation, our way of constructing query-dependent table-passage chains is likely to improve the density of relevant information for single-hop questions.

For the OTT-QA chains, there is little overlap between the question and the target entity passage as expected.
Thus, it is relatively difficult for the retriever to succeed in gathering all relevant information alone.
On the contrary, our framework can effectively handle it with our proposed linking and chaining operations.   

==> EMNLP 2022/7-Related-work.tex <==
\section{Related Work}
Multi-hop question answering (QA) has been studied extensively for both knowledge base (KB) setting \cite{yih-etal-2015-semantic,zhang2017variational,talmor-berant-2018-web} and open-domain setting \cite{yang-etal-2018-hotpotqa,feldman-el-yaniv-2019-multi,geva-etal-2021-aristotle}. For KB-based setting, the models are trained to parse questions into logical forms that can be executed against KB \cite{das-etal-2021-case,yu2022decaf} or directly select entities in KB as answers \cite{sun-etal-2019-pullnet}. On the other hand, the open-domain setting requires the model to retrieve multiple pieces of evidence from a textual corpus and then produce the answer \cite{nie-etal-2019-revealing,zhu-etal-2021-adaptive}. Our work falls into the latter category.  

One stream of open-domain work uses multiple rounds of retrieval, where the later rounds depend on the previous ones.
It is typically achieved by some form of query reformulation, \eg expanding the question with previous passages \cite{xiong2020answering,zhao-etal-2021-multi-step} or re-writing the query using relevant evidence keywords \cite{qi-etal-2019-answering,qi-etal-2021-answering}.
The other line of work directly leverages the gold graph structure to expand the initial set of passages for hopping \cite{ding-etal-2019-cognitive,asai2019learning,10.1145/3404835.3462942}, assuming the presence of oracle hyperlinks.  
Different from those customized text-only multi-hop methods, our approach constructs evidence graphs on-the-fly and we show that it can handle single/multi-hop questions with a unified model over heterogeneous knowledge sources. Moreover, we do not presume the existence of gold hyperlinks in the corpus, making our model more applicable in realistic settings. 
% Multi-hop QA over knowledge bases has also been studied extensively in the literature .
% Given its structured nature of KB, recent multi-hop QA methods focus on enriching the representation of KB symbols with text, such as using text retrieval for ranking \cite{sun-etal-2019-pullnet,dhingra2020differentiable} or embedding KB facts using language models \cite{verga2020facts}.
% Other efforts have attempted to embed KB facts or entities as memory of the language models \cite{verga2020facts}, and leverage this encoded knowledge with graph neural networks for QA \cite{yu2020jaket}. 

There are also recent efforts in leveraging structured knowledge for ODQA.
\citet{li-etal-2021-dual} proposed to leverage information from both text and tables to generate answers and SQL queries.
\citet{oguz2020unikqa} studied the benefits of both tables and knowledge bases on a set of ODQA tasks.
\citet{ma-etal-2022-open} introduced a unified knowledge interface that first verbalizes tables and KB sub-graphs into text and then uses a single retriever-reader model to handle all knowledge sources. 
Similarly, we also consider heterogeneous knowledge sources for ODQA.
Instead of developing task-specific models and considering the evidence in isolation, we focus on finding evidence paths across different knowledge types for single/multi-hop questions.

% Our work differs from those previous works in the following aspects: we propose dedicated intermediary modules to construct evidence graphs and find query dependent paths, which do not assume any pre-existing link annotation: e.g. hyperlinks; our framework can effectively find evidence chains across different types of knowledge, and a single unified model can learn to solve both single-hop and multi-hop tasks under our framework. 

==> EMNLP 2022/8-Conclusions.tex <==
\section{Conclusion}
In this paper, we present a new framework, \ourmodel, for ODQA over heterogeneous knowledge sources.
With the novel task-agnostic intermediary module, \ourmodel~can effectively handle single/multi-hop tasks using a unified model and achieve new SOTA results on OTT-QA.
Our analyses show that the intermediary module is necessary to achieve good results. 
%\chenghao{I guess future work can all go to limitations?}
%For future work, it would be interesting to study other instantiation of our framework, e.g. a more generic linker that is able to build other types of edges including passage-to-passage, passage-to-knowledge-base, etc. 
For future work, it would be interesting to apply our framework to other complex reasoning tasks such as fact verification \cite{thorne-etal-2018-fever,aly2021feverous} or commonsense QA \cite{talmor2022commonsenseqa}. % Most recently, \citet{zhong2022reasoning} proposed to pretrain a evidence chain extractor to find the answer cues across tables and passages. 
\clearpage


==> EMNLP 2022/9-Limitations.tex <==
\section{Limitations}
We identify the limitations of our study below.

Conceptually, our proposed linker model is generic and it should be able to build edges between documents regardless of their type, e.g. passage-to-passage, passage-to-table. However, in this paper, we focus on one instantiation of the linker model, linking tables to passages. It would be interesting to build a more generic linker that is able to handle different edge types. 

Although we have experimented with OTT-QA and NQ, which exhibit very different question styles and reasoning types, both tasks are built on Wikipedia.
As most pretrained language models used in our work are also trained using Wikipedia, there are potential issues in generalization.
It would be interesting to apply our framework to other domains and test its generalizability, \eg biomedical domain. 

One major bottleneck we found in our experiments is computation. Since we use the T0-3B model (which is the cheaper one, T0-11B is the recommended model by \citet{sanh2021multitask}) as our chainer, it incurs a very large memory footprint and computation cost even just for inference.
Moreover, the FiD reader model is built on T5-large. Encoding top-50 chains is still computationally expensive.
In our case, even with a per GPU batch size of 1, the model still cannot run on V100-32G GPUs, thus we had to resort to gradient checkpointing, leading to longer running time.
It would be interesting to experiment with other alternatives that require less computation. 

% Finally, we note that both the datasets and the models we used are English-only. As there are thousands of other languages in the world, it would be worth applying our framework to other language settings, or building a multi-lingual system, which would make a larger impact and have much broader applications in real-world scenarios. 

==> EMNLP 2022/Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}


\newcommand{\R}{\mathbb{R}}

\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mR}{\mathcal{R}}

\newcommand{\iL}{\mathit{L}}
\newcommand{\iQ}{\mathit{Q}}
\newcommand{\iR}{\mathit{R}}
\newcommand{\iU}{\mathit{U}}
\newcommand{\iV}{\mathit{V}}
\newcommand{\iX}{\mathit{X}}
\newcommand{\iY}{\mathit{Y}}

\newcommand{\sigmoid}{\text{sigm}}
%\newcommand{\vector}{\text{vec}}
\newcommand{\KL}{\text{KL}}
\newcommand{\Loss}{\mathcal{L}}
% \newcommand{\st}{\text{ s.t. }}

% Objective functions
\newcommand{\bilinear}[3]{#1^{\top}#2#3}
\newcommand{\bidiag}[3]{(#1 \circ #3) ^{\top} #2}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\biband}[3]{#1^{\top}#2#3}

% Dependency paths
\newcommand{\leftarc}[1]{$\leftarrow${[#1]}-}
\newcommand{\rightarc}[1]{-{[#1]}$\rightarrow$}
\newcommand{\wildcard}{$\langle*\rangle$}

\newcommand{\gene}[1]{{\texttt{#1}}}
\newcommand{\rev}[1]{#1$^{-1}$}

\newcommand{\neigh}[1]{\text{nb}\left(#1\right)}
\newcommand{\diagm}[1]{\text{diag}\left(#1\right)}
\newcommand{\ind}[1]{\mathbf{1}\left(#1\right)}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
%\newcommand{\vector}[1]{\underset{#1}{\text{vec}}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\newcommand{\cheading}[2]{\textbf{#1\hfill #2}}
\newcommand{\highest}[1]{\textbf{#1}}% == highest score



%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
% \newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.3mm]}
\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\etc}{\emph{etc.}\ }
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.,}\ }
\newcommand{\ie}{\emph{i.e.,}\ }
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\rhs}{\text{ r.h.s. }}
\newcommand{\lhs}{\text{ l.h.s. }}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\tauvec}{\vec{\tau}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
\newcommand{\Img}{\ensuremath{\mathrm{Im}}}

\newcommand{\cvxCondjc}{{\sf cvxCondJC}}
\newcommand{\cvxCond}{{\sf cvxCond}}
\newcommand{\altCondjc}{{\sf altCondJC}}
\newcommand{\altCond}{{\sf altCond}}

\newcommand{\cvxDisc}{{\sf cvxDisc}}
\newcommand{\JB}{{\sf JB}}
\newcommand{\GS}{{\sf GS}}

\newcommand{\cvxJoint}{{\sf cvxJoint}}
\newcommand{\LG}{{\sf LG}}
\newcommand{\NB}{{\sf NB}}

%%%%%%%%%%%%%%%%%%%linear algebra defs%%%%%%%%%%%%%%%
\newcommand{\unifint}{\int^{1}_{0}}


==> EMNLP 2022/intro_v2.tex <==
\begin{comment}
Reasoning in real-world scenarios, such as open-domain question answering (ODQA), typically requires a chain of compositional steps.
Consider the question in \autoref{fig:model}.
To form the final answer, a model needs to find the entry list of the mentioned touring car race in 1995, look up the driver name with the correct rank, search for the corresponding driver information, and extract the birthplace.
\chenghao{Makes this more concrete, something should stand out here: multi-hop evidence gathering across different types of knowledge sources.}
% Complex question answering tasks that require multi-step compositional reasoning are often used to test model's ability to understand natural language \cite{}.
% Move this to related work.
% For multi-hop reasoning against text, one popular approach is to decompose the complex question into a sequence of simple sub-questions and infer the final answer based on simpler questions \cite{perez-etal-2020-unsupervised,wolfson-etal-2020-break}.
There are two popular paradigms for tackling this challenge. 
% For structured or semi-structured knowledge sources, semantic parsing techniques, mapping natural language question into executable programs, have been long researched for compositional question understanding \cite{}.
% add John M Zelle and Raymond J Mooney. Learning to parse database queries using inductive logic programming. In Proceedings of the national conference on artificial intelligence, 1996
% Luke S Zettlemoyer and Michael Collins. Learning to map sentences to logical form: structured classification with probabilistic categorial grammars. In UAI ’05, 2005.
The neuro-symbolic paradigm first parses complex questions into discrete operations and then assembles 
corresponding neural modules to complete the \textit{symbolic reasoning} against various knowledge sources \cite{Gupta2020NeuralMN,jiang-bansal-2019-self,andreas-etal-2016-learning}.
The other paradigm fully leverages the pretrained language models (PLMs) for reasoning solely in natural language,
tapping into the implicit knowledge of PLMs rather than relying on a closed set of task-specific operations.
% Instead of relying on a task-dependent set of operations/symbols (``closed world'' settings), another recent line of work fully leverages the pretrained language models (PLMs) for reasoning solely in natural language (i.e. tapping into the implicit knowledge of PLMs for reasoning).
Specifically, most \textit{PLM-based reasoning} approaches focus on eliciting the PLMs to carry out multi-step reasoning via explicit knowledge prompts, such as real-world facts \cite{talmor2020leap-of-thought} and human-written step-by-step inference demonstrations \cite{wei-el-al-2022-chain-of-thought}.
% such as teaching the model to use generated rules \cite{talmor2020leap-of-thought} or prompting the model to mimic the carefully human written reasoning steps \cite{wei-el-al-2022-chain-of-thought}. However, the success of these approaches are largely achieved on well-controlled synthetic or domain-specific settings without the capability to reason against open-domain heterogeneous knowledge sources.
\end{comment}


\begin{comment}
Motivated by their success in synthetic cases, we aim to enhance the PLM-based reasoning with interpretable discrete operations against open-domain heterogeneous knowledge sources.
Specifically, we propose the \textbf{C}hain \textbf{O}f \textbf{RE}asoning (\ourmodel) framework %a general PLM-based open-domain reasoning framework 
\chenghao{How about core, which can be pronounced by more easily?}
\eric{CoR sounds better} consisting of three generic operations \eric{(Maybe "four discrete steps/modules/algorithms") formalizing the idea of using linking and chaining in open-domain reasoning}: finding relevant evidences (retrieval), piecing related reasons together (linking \& chaining), and producing answers using explicit chains of reasons (reading).
Our framework can be viewed as the synergy between symbolic reasoning (discrete operations) and PLM-based reasoning (PLM-based reader). 
Similar to symbolic reasoning, our approach can achieve better explainability via explicit steps of chaining reasons together and thus mitigate the well-known hallucination issue of PLMs \cite{}.
At the same time, our discrete operations are generic enough to be useful for more real-world open-domain applications than those task-specific cases considered by previous work.
% In this paper, we propose a generalizable framework for reasoning in open-domain setting that combines the strengths from both streams of approaches. Instead of fully replying on the PLM to figure out all reasoning steps (finding reasons, chaining reasons, and grounding on proper reasons to form answers/conclusions), we decompose these into two steps, where the finding reasons and chaining them are discrete operations (explicit part) and the LM only performing the last grounded reasoning step (implicit part).
% This can achieve more trustworthy explainability compare to black-box models that fully relies on the implicit knowledge of PLMs \cite{roberts-etal-2020-much,NEURIPS2020_1457c0d6}, likely resulting in hallucination.
%as the individual/chained reasons are not generated as in \citet{talmor2020leap-of-thought}.
% At the same time, our approach does not reply on humans to manually craft thoughts for prompting LMs, potentially making it more scalable and useful for more open-domain reasoning with available knowledge sources.
\end{comment}

The task of open-domain question answering typically requires multi-hop reasoning, finding relevant individual evidences from external knowledge sources, piecing related evidences with context together, and then producing answers based on the final supportive evidence set.
While many questions can be answered by a single piece of evidence \cite{joshi-etal-2017-triviaqa,kwiatkowski-etal-2019-natural},
answering more complex questions are of great interest as it requires reasoning beyond \textit{local} document context \cite{yang-etal-2018-hotpotqa, geva-etal-2021-aristotle}. The problem becomes even more challenging when the required evidence are scattered across heterogeneous sources, e.g. unstructured text vs structured tables \cite{chen2020open} (hopping from one modality of knowledge to another). 
Consider the question in \autoref{fig:model}.
To form the final answer, a model needs to find the entry list (a table) of the mentioned touring car race, look up the driver name with the correct rank, search for the corresponding driver information, and extract the birthplace in the free text.

However, existing methods on ODQA largely customize the retriever-reader model for tackling single-hop or multi-hop questions separately.
In other words, they exclusively rely on the retriever to gather all necessary context in a query-dependent fashion.
For single-hop questions, the retriever only fetches a list of isolated passages (dots) \cite{karpukhin-etal-2020-dense}.
For multi-hop questions, an iterative retriever is used to find a query-dependent path of passages (chains) \cite{xiong2020answering}, i.e. the later hop passages are retrieved using an expanded query including the original question and all previous hop passages.
Although those separate treatments achieve promising results on their targeted cases, the customized retrievers are unable to generalize well.
For example, an iterative retriever trained with both multi-hop and single-hop questions performs poorly over either types of questions \cite{xiong2020answering}.
For real-word applications, it is desirable for an ODQA system to handle both cases reasonably well.
% potentially due to the discrepancy of inputs between hops. 








%Previous works on ODQA adopts different modeling methods for solving single-hop or multi-hop questions. For single-hop questions, the model only retrieve once over the document index and the Top-K returned documents are processed by the reader \cite{karpukhin-etal-2020-dense}. Whereas for multi-hop questions, the retriever runs multiple times using the question and documents returned in previous rounds as query, to find the complete reasoning chains \cite{xiong2020answering}. While these methods achieve promising results on their targeted problem sets, they can not generalize well to other types of questions.  

%In this paper, we propose a novel framework that unifies the solutions for single hop and multi-hop questions over heterogeneous sources. In particular, we first build a bipartite graph between different knowledge sources, then our retriever run inference only on one of the knowledge source and we expand the retrieved documents using the edges in the bipartite graph, therefore completing the reasoning chain for multi-hop questions. Our reader then jointly reason over the linked evidences to find the final answer. We evaluated our framework on the multi-hop dataset OTT-QA \cite{chen2020open} and single-hop dataset NQ \cite{kwiatkowski-etal-2019-natural}. Our method achieves the state-of-the-art results on OTT-QA by outperforming the previous SOTA by 14+ points on exact match score, which is over 40\% relative gains. 

==> intro_v2.tex <==
\begin{comment}
Reasoning in real-world scenarios, such as open-domain question answering (ODQA), typically requires a chain of compositional steps.
Consider the question in \autoref{fig:model}.
To form the final answer, a model needs to find the entry list of the mentioned touring car race in 1995, look up the driver name with the correct rank, search for the corresponding driver information, and extract the birthplace.
\chenghao{Makes this more concrete, something should stand out here: multi-hop evidence gathering across different types of knowledge sources.}
% Complex question answering tasks that require multi-step compositional reasoning are often used to test model's ability to understand natural language \cite{}.
% Move this to related work.
% For multi-hop reasoning against text, one popular approach is to decompose the complex question into a sequence of simple sub-questions and infer the final answer based on simpler questions \cite{perez-etal-2020-unsupervised,wolfson-etal-2020-break}.
There are two popular paradigms for tackling this challenge. 
% For structured or semi-structured knowledge sources, semantic parsing techniques, mapping natural language question into executable programs, have been long researched for compositional question understanding \cite{}.
% add John M Zelle and Raymond J Mooney. Learning to parse database queries using inductive logic programming. In Proceedings of the national conference on artificial intelligence, 1996
% Luke S Zettlemoyer and Michael Collins. Learning to map sentences to logical form: structured classification with probabilistic categorial grammars. In UAI ’05, 2005.
The neuro-symbolic paradigm first parses complex questions into discrete operations and then assembles 
corresponding neural modules to complete the \textit{symbolic reasoning} against various knowledge sources \cite{Gupta2020NeuralMN,jiang-bansal-2019-self,andreas-etal-2016-learning}.
The other paradigm fully leverages the pretrained language models (PLMs) for reasoning solely in natural language,
tapping into the implicit knowledge of PLMs rather than relying on a closed set of task-specific operations.
% Instead of relying on a task-dependent set of operations/symbols (``closed world'' settings), another recent line of work fully leverages the pretrained language models (PLMs) for reasoning solely in natural language (i.e. tapping into the implicit knowledge of PLMs for reasoning).
Specifically, most \textit{PLM-based reasoning} approaches focus on eliciting the PLMs to carry out multi-step reasoning via explicit knowledge prompts, such as real-world facts \cite{talmor2020leap-of-thought} and human-written step-by-step inference demonstrations \cite{wei-el-al-2022-chain-of-thought}.
% such as teaching the model to use generated rules \cite{talmor2020leap-of-thought} or prompting the model to mimic the carefully human written reasoning steps \cite{wei-el-al-2022-chain-of-thought}. However, the success of these approaches are largely achieved on well-controlled synthetic or domain-specific settings without the capability to reason against open-domain heterogeneous knowledge sources.
\end{comment}


\begin{comment}
Motivated by their success in synthetic cases, we aim to enhance the PLM-based reasoning with interpretable discrete operations against open-domain heterogeneous knowledge sources.
Specifically, we propose the \textbf{C}hain \textbf{O}f \textbf{RE}asoning (\ourmodel) framework %a general PLM-based open-domain reasoning framework 
\chenghao{How about core, which can be pronounced by more easily?}
\eric{CoR sounds better} consisting of three generic operations \eric{(Maybe "four discrete steps/modules/algorithms") formalizing the idea of using linking and chaining in open-domain reasoning}: finding relevant evidences (retrieval), piecing related reasons together (linking \& chaining), and producing answers using explicit chains of reasons (reading).
Our framework can be viewed as the synergy between symbolic reasoning (discrete operations) and PLM-based reasoning (PLM-based reader). 
Similar to symbolic reasoning, our approach can achieve better explainability via explicit steps of chaining reasons together and thus mitigate the well-known hallucination issue of PLMs \cite{}.
At the same time, our discrete operations are generic enough to be useful for more real-world open-domain applications than those task-specific cases considered by previous work.
% In this paper, we propose a generalizable framework for reasoning in open-domain setting that combines the strengths from both streams of approaches. Instead of fully replying on the PLM to figure out all reasoning steps (finding reasons, chaining reasons, and grounding on proper reasons to form answers/conclusions), we decompose these into two steps, where the finding reasons and chaining them are discrete operations (explicit part) and the LM only performing the last grounded reasoning step (implicit part).
% This can achieve more trustworthy explainability compare to black-box models that fully relies on the implicit knowledge of PLMs \cite{roberts-etal-2020-much,NEURIPS2020_1457c0d6}, likely resulting in hallucination.
%as the individual/chained reasons are not generated as in \citet{talmor2020leap-of-thought}.
% At the same time, our approach does not reply on humans to manually craft thoughts for prompting LMs, potentially making it more scalable and useful for more open-domain reasoning with available knowledge sources.
\end{comment}

The task of open-domain question answering typically requires multi-hop reasoning, finding relevant individual evidences from external knowledge sources, piecing related evidences with context together, and then producing answers based on the final supportive evidence set.
While many questions can be answered by a single piece of evidence \cite{joshi-etal-2017-triviaqa,kwiatkowski-etal-2019-natural},
answering more complex questions are of great interest as it requires reasoning beyond \textit{local} document context \cite{yang-etal-2018-hotpotqa, geva-etal-2021-aristotle}. The problem becomes even more challenging when the required evidence are scattered across heterogeneous sources, e.g. unstructured text vs structured tables \cite{chen2020open} (hopping from one modality of knowledge to another). 
Consider the question in \autoref{fig:model}.
To form the final answer, a model needs to find the entry list (a table) of the mentioned touring car race, look up the driver name with the correct rank, search for the corresponding driver information, and extract the birthplace in the free text.

However, existing methods on ODQA largely customize the retriever-reader model for tackling single-hop or multi-hop questions separately.
In other words, they exclusively rely on the retriever to gather all necessary context in a query-dependent fashion.
For single-hop questions, the retriever only fetches a list of isolated passages (dots) \cite{karpukhin-etal-2020-dense}.
For multi-hop questions, an iterative retriever is used to find a query-dependent path of passages (chains) \cite{xiong2020answering}, i.e. the later hop passages are retrieved using an expanded query including the original question and all previous hop passages.
Although those separate treatments achieve promising results on their targeted cases, the customized retrievers are unable to generalize well.
For example, an iterative retriever trained with both multi-hop and single-hop questions performs poorly over either types of questions \cite{xiong2020answering}.
For real-word applications, it is desirable for an ODQA system to handle both cases reasonably well.
% potentially due to the discrepancy of inputs between hops. 








%Previous works on ODQA adopts different modeling methods for solving single-hop or multi-hop questions. For single-hop questions, the model only retrieve once over the document index and the Top-K returned documents are processed by the reader \cite{karpukhin-etal-2020-dense}. Whereas for multi-hop questions, the retriever runs multiple times using the question and documents returned in previous rounds as query, to find the complete reasoning chains \cite{xiong2020answering}. While these methods achieve promising results on their targeted problem sets, they can not generalize well to other types of questions.  

%In this paper, we propose a novel framework that unifies the solutions for single hop and multi-hop questions over heterogeneous sources. In particular, we first build a bipartite graph between different knowledge sources, then our retriever run inference only on one of the knowledge source and we expand the retrieved documents using the edges in the bipartite graph, therefore completing the reasoning chain for multi-hop questions. Our reader then jointly reason over the linked evidences to find the final answer. We evaluated our framework on the multi-hop dataset OTT-QA \cite{chen2020open} and single-hop dataset NQ \cite{kwiatkowski-etal-2019-natural}. Our method achieves the state-of-the-art results on OTT-QA by outperforming the previous SOTA by 14+ points on exact match score, which is over 40\% relative gains. 
